Variational measurement-based quantum computation for generative modeling

Measurement-based quantum computation (MBQC) offers a fundamentally unique paradigm to design quantum algorithms. Indeed, due to the inherent randomness of quantum measurements, the natural operations in MBQC are not deterministic and unitary, but are rather augmented with probabilistic byproducts. Yet, the main algorithmic use of MBQC so far has been to completely counteract this probabilistic nature in order to simulate unitary computations expressed in the circuit model. In this work, we propose designing MBQC algorithms that embrace this inherent randomness and treat the random byproducts in MBQC as a resource for computation. As a natural application where randomness can be beneficial, we consider generative modeling, a task in machine learning centered around generating complex probability distributions. To address this task, we propose a variational MBQC algorithm equipped with control parameters that allow one to directly adjust the degree of randomness to be admitted in the computation. Our algebraic and numerical findings indicate that this additional randomness can lead to significant gains in expressivity and learning performance for certain generative modeling tasks, respectively. These results highlight the potential advantages in exploiting the inherent randomness of MBQC and motivate further research into MBQC-based algorithms.

==> recommendations.tex <==
% \noindent\textbf{Recommendation 1 @Arun and @Tina}:\\ 
% Maintain a \textbf{single .bib} for all your publication as it will help you tremendously in the future writing of papers and your thesis. 
% Also maintain a standardized way of labelling references. Personally, I like "last name of first author - year - first word of title", e.g. "raussendorf2001a" for Ref.~\cite{raussendorf2001a}\\

% \noindent\textbf{Recommendation 2 @Arun and @Tina}:\\ 
% Do not start with the results section. \textbf{Start with the background material} and something like a "Related Work" section (here, Methods). That is, first contextualize your work w.r.t. prior research in the field. Only when you can clearly distinguish yourself from the rest of the scientific literature should you start with the results. The introduction can also help putting this work into context and establishing a storyline.\\

% \noindent\textbf{Recommendation 3 @Arun and @Tina}:\\ 
% Do not immediately write a flowing text. Instead, make an \textbf{itemized list} with the content for each section.\\

% \noindent\textbf{Recommendation 4 @Arun and @Tina}:\\ 
% For quick and dirty writing and collaborating, I do not like using the in-built overleaf tool for commenting. Instead, I like using colors to indicate a comment from \hpn{me}. You can also use your names to add colors to your writing \arun{@Arun}, \tina{@Tina} (see bottom of "definitions.tex" file).
